Action-based distribution function modelling for constraining the shape of the Galactic dark matter halo

We estimate the 3D density profile of the Galactic dark matter (DM) halo within $r \lesssim 30$ kpc from the Galactic centre by using the astrometric data for halo RR Lyrae stars from Gaia DR2. We model both the stellar halo distribution function and the Galactic potential, fully taking into account the survey selection function, the observational errors, and the missing line-of-sight velocity data for RR Lyrae stars. With a Bayesian MCMC method, we infer the model parameters, including the density flattening of the DM halo $q$, which is assumed to be constant as a function of radius. We find that 99\% of the posterior distribution of $q$ is located at $q>0.963$, which strongly disfavours a flattened DM halo. We cannot draw any conclusions as to whether the Galactic DM halo at $r \lesssim 30$ kpc is prolate, because we restrict ourselves to axisymmetric oblate halo models with $q\leq1$. Our result is inconsistent with predictions from cosmological hydrodynamical simulations that advocate more oblate ($\langle{q}\rangle \sim0.8 \pm 0.15$) DM halos within $\sim 15\%$ of the virial radius for Milky-Way-sized galaxies. An alternative possibility, based on our validation tests with a cosmological simulation, is that the true value $q$ of the Galactic halo could be consistent with cosmological simulations but that disequilibrium in the Milky Way potential is inflating our measurement of $q$ by 0.1-0.2. As a by-product of our analysis, our model constrains the DM density in the Solar neighbourhood to be $\rho_{\mathrm{DM},\odot} = (9.01^{+0.18}_{-0.20})\times10^{-3}M_\odot \mathrm{pc}^{-3} = 0.342^{+0.007}_{-0.007}$ $\;\mathrm{GeV} \mathrm{cm}^{-3}$.

==> table1.tex <==
\begin{table}
\centering
\caption{ {\tableOneCaption} }
\label{tab:prior}
\begin{tabular}{lll} % four columns, alignment for each
\hline
Quantity & Prior probability distribution & Note\\
\hline
\hline 
$M_\mathrm{bulge}$ & $M_\mathrm{bulge} = (8.9\pm0.89) \times 10^9 M_\odot$ &   \\
$R_\mathrm{d}^\mathrm{thin}$  & $R_\mathrm{d}^\mathrm{thin}= (2.6\pm0.52) \kpc$  & \\
$R_\mathrm{d}^\mathrm{thick}$ & $R_\mathrm{d}^\mathrm{thick}= (3.6\pm0.72) \kpc$  & \\
$\Sigma_0^\mathrm{thin}$  & Flat at $0 < \Sigma_0^\mathrm{thin} $  & \\
$\Sigma_0^\mathrm{thick}$ & Flat at $0 < \Sigma_0^\mathrm{thick}$  & \\
$q$ & Flat at $0.2 < U \leq 0.5$ (oblate) & (1) \\
$\gamma$ & Flat at $0 < \gamma < 1.9$ &  \\
$\log_{10} a$ & Flat at $-\infty < \log_{10} a < \infty$ &  \\
$\log_{10} \rho_0$ & Flat at $-\infty < \log_{10} \rho_0 <\infty$ &  \\
Thick to thin disk ratio  & $f_{\mathrm{d, \odot}}=(0.12\pm0.012)$ & (2)\\
Total stellar mass & Equation (\ref{eq:stellarMass}) & (2) \\
Dark matter concentration & $\ln c'_\mathrm{v} = 2.56 \pm 0.272$ & (2) \\
%$(R_\mathrm{d}^\mathrm{thin}, R_\mathrm{d}^\mathrm{thick}, \Sigma_0^\mathrm{thin}, \Sigma_0^\mathrm{thick})$ & $f_{\mathrm{d, \odot}}=(0.12\pm0.012)$ & (1)\\
\hline 
$(h_r, h_z, h_\phi)$ & Equation (\ref{eq:hgprior}) & (2) \\
$(g_r, g_z, g_\phi)$ & Equation (\ref{eq:hgprior}) & (2) \\
$\log_{10} J_0$ & Flat at $-\infty  < \log_{10} J_0 < \infty $ &  \\
$\Gamma$  & Flat at $0 \leq \Gamma < 2.8$ & \\
$B$       & Fixed to $B=5$ &  \\
$\log_{10} \eta$ & Flat at $-\infty < \log_{10} \eta < -2$ &  \\
\hline 
\end{tabular} \\
\flushleft{\tableOneNote}
\end{table}


